Generative Control of Time-Modulated Intelligent Reflecting Surfaces for Scalable Directional Modulation

Time-modulated intelligent reflecting surfaces (TM-IRS) achieve directional modulation by switching their elements on and off at designed instants and durations, so that an undistorted signal reaches the intended user while appearing scrambled elsewhere. We propose a Flow Matching (FM)-based generative framework that designs these parameters for strong scrambling and reliable reception simultaneously. For orthogonal frequency-division multiplexing (OFDM) signals, we introduce a physics-informed reward that maximizes the time-modulation harmonic energy radiated in the null space of the legitimate-user response, subject to a minimum per-subcarrier signal-to-interference-plus-noise ratio (SINR), without requiring knowledge of adversary directions. Unlike prior generative flow network (GFlowNet) approaches, which assign discretized parameters sequentially, the FM model generates complete continuous configurations jointly, decoupling the generation depth from the number of elements and accelerating training. It also learns a distribution over configurations that can be resampled to vary the scrambling pattern. Numerical results show that, compared with a GFlowNet baseline, the proposed approach reduces the time to training loss near-saturation by $99.4\%$ on average for $3{\times}3$ to $12{\times}12$ surfaces, attains higher final rewards, scales to $80{\times}80$, and confines the low-symbol-error region more tightly around the legitimate user.

==> Format.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Packages to Load
%% Text and Math Environment Packages
\RequirePackage{csquotes} %Package to Facilities Quotations
% \RequirePackage[backend=biber, style=ieee, sorting=ynt]{biblatex} % Conflict with IEEE reference formating
\RequirePackage[noadjust]{cite} % IEEE uses this
% \RequirePackage[english]{babel} % Do not use with IEEE, causing wrong figure naming
% \RequirePackage[utf8]{inputenc} %utf8 Support. Preloaded in Distribution
\RequirePackage[T1]{fontenc} %Better Font Encoding for T1 Type Font
\RequirePackage[shortlabels, inline]{enumitem} %Conflict with Beamer
\RequirePackage[table, svgnames]{xcolor} %Beamer Has This by Default
\RequirePackage[most]{tcolorbox} %Customized Box. Must Load after xcolor
\RequirePackage{mathtools} %Customize Math Symbols and Theorems
\RequirePackage{amsthm} %Theorem environments
% \RiquirePackage{amsmath} %Loaded by mathtools
\RequirePackage{amssymb} %Conflict with Fonts
% \RequirePackage{Fonts} %Must Load after tcolorbox and amsthm
% \let\openbox\undefined %Fix Some Font Issues
\RequirePackage{mleftright} %Fixes Some Math Spacing Issues
\RequirePackage{siunitx}
\RequirePackage{bm} %Boldface Math, Load after Other Math Font Packages
\RequirePackage{microtype} %Better Font Spacing
\RequirePackage[normalem]{ulem} %Underlining and strikeout support
\RequirePackage{fontawesome5} %

%% Table Packages
\RequirePackage{tabularx} %Including Tabular with More Space Option
% \RequirePackage{colortbl} %Package to Use Color in Tables. Replaced by table option of xcolor
\RequirePackage{multirow} %Package to Use Multirow in Tables
\RequirePackage{multicol} %Package to Use Multicols
\RequirePackage{array} %Math and More Spacing Support in Tables

%% Graphics Packages
\RequirePackage{epstopdf} %Package to Convert EPS to PDF in PDFLaTeX
\RequirePackage{transparent} %Transparent Images
\RequirePackage{graphicx} %Graphics Backend with key-value Arguments
\RequirePackage[export]{adjustbox} %More Arguments for includegraphics
\RequirePackage[caption=false, font=footnotesize]{subfig} % IEEE uses subfig instead of subcaption

%% IEEE Figure Style
% \makeatletter
% \let\MYcaption\@makecaption
% \makeatother

% \RequirePackage[font=footnotesize]{subcaption}

% \makeatletter
% \let\@makecaption\MYcaption
% \makeatother

%% Code Packages
% \RequirePackage{listings} %Loaded by tcolorbox and also no need of minted.
\RequirePackage{algorithm} %Package to Insert Algorithm
\RequirePackage{algpseudocode} %Package to Insert Algorithm

%% Other Packages
\RequirePackage{xspace} %Package to Add Space after Macros
% \RequirePackage{calc} %Package of Calculation in Latex
% \RequirePackage{rotating} %Package to Rotate Objects
% \RequirePackage{pgf, tikz} %Package to Draw Figures.
% \RequirePackage{keyval} %Package to Enable Key-val syntex
\RequirePackage{hyperref} %Beamer Has This by Default.
\RequirePackage{bookmark}
\RequirePackage{orcidlink}
\RequirePackage[capitalise,nameinlink]{cleveref} %Must Load after others. Conflict with Beamer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

